The POLARBEAR-2 and Simons Array Focal Plane Fabrication Status

We present on the status of POLARBEAR-2 A (PB2-A) focal plane fabrication. The PB2-A is the first of three telescopes in the Simon Array (SA), which is an array of three cosmic microwave background (CMB) polarization sensitive telescopes located at the POLARBEAR (PB) site in Northern Chile. As the successor to the PB experiment, each telescope and receiver combination is named as PB2-A, PB2-B, and PB2-C. PB2-A and -B will have nearly identical receivers operating at 90 and 150 GHz while PB2-C will house a receiver operating at 220 and 270 GHz. Each receiver contains a focal plane consisting of seven close-hex packed lenslet coupled sinuous antenna transition edge sensor bolometer arrays. Each array contains 271 di-chroic optical pixels each of which have four TES bolometers for a total of 7588 detectors per receiver. We have produced a set of two types of candidate arrays for PB2-A. The first we call Version 11 (V11) and uses a silicon oxide (SiOx) for the transmission lines and cross-over process for orthogonal polarizations. The second we call Version 13 (V13) and uses silicon nitride (SiNx) for the transmission lines and cross-under process for orthogonal polarizations. We have produced enough of each type of array to fully populate the focal plane of the PB2-A receiver. The average wirebond yield for V11 and V13 arrays is 93.2% and 95.6% respectively. The V11 arrays had a superconducting transition temperature (Tc) of 452 +/- 15 mK, a normal resistance (Rn) of 1.25 +/- 0.20 Ohms, and saturations powers of 5.2 +/- 1.0 pW and 13 +/- 1.2 pW for the 90 and 150 GHz bands respectively. The V13 arrays had a superconducting transition temperature (Tc) of 456 +/-6 mK, a normal resistance (Rn) of 1.1 +/- 0.2 Ohms, and saturations powers of 10.8 +/- 1.8 pW and 22.9 +/- 2.6 pW for the 90 and 150 GHz bands respectively.

==> references.tex <==

\begin{thebibliography}{99}

\bibitem{AdvancedAct}
S. W. Henderson et. al, {\it J. Low Temp. Phys.} \textbf{184}, 3-4, (2016), DOI: 10.1007/s10909-016-1575-z

\bibitem{BICEP1_2008}
Yuki D. Takahashi et. al., {\it SPIE Proceedings} \textbf{7020}, 12, (2008), DOI: 10.1117/12.790306/SPIE

\bibitem{BICEP2Keck_Planck_JointAnalysis}
BICEP2/Keck Collaboration \and Planck Collaboration, {\it PhRvL}, \textbf{114}, 10, (2015), DOI: 10.1103/PhysRevLett.114.101301

\bibitem{BICEP3_2016}	
W. L. K. Wu et. al, {\it J. Low Temp. Phys.}, \textbf{184} 3-4, (2016), DOI: 10.1007/s10909-015-1403-x

\bibitem{POLARBEAR1_2012}
The POLARBEAR Collaboration, {\it SPIE Proceedings} \textbf{8452}, 15, (2012), DOI: 10.1117/12.926354/SPIE

\bibitem{POLARBEAR2_2016}
The POLARBEAR Collaboration, {\it SPIE Proceedings} \textbf{9914}, 9, (2016), DOI: 	10.1117/12.2231961/SPIE

\bibitem{POLARBEAR2_LTD}
The POLARBEAR Collaboration, {\it J. Low Temp. Phys.} \textbf{184}, 3-4, (2016), DOI: 10.1007/s10909-015-1425-4

\bibitem{POLARBEAR2_Readout}
The POLARBEAR Collaboration, {\it J. Low Temp. Phys.} \textbf{},

\bibitem{POLARBEAR_LensingBmodes}
The POLARBEAR Collaboration, {\it ApJ} \textbf{794}. 171, (2014), DOI: 10.1088/0004-637X/794/2/171

\bibitem{SPTPOL1_2012}
J.~E. Austermann et. al., {\it SPIE Proceedings} \textbf{8452}, 18, (2012), DOI: 10.1117/12.927286/SPIE

\bibitem{SPTPOL3G_2014}
B.~A. Benson et. al., {\it SPIE Proceedings} \textbf{9153}, 21, (2014), DOI: 10.1117/12.2057305/SPIE

\bibitem{SPTPol_LensingBmodes}
Hanson, D. et. al., {\it PhRvL} \textbf{111}, 14, (2013), DOI: 10.1103/PhysRevLett.111.141301

\bibitem{Dobbs_DfMUX},
Dobbs, M. et. al., {\it IEEE Transactions on Nuclear Science}, 55,  (2008), DOI: 10.1109/TNS.2007.911601

\bibitem{Westbrook_Sinuous},
Westbrook, B. et. al. {\it JTLP}, 184, (2016), pp74--81

\bibitem{PB2_Readout},
Elleflot, Tucker et. al. {\it JTLP, in review}, (2018)



\end{thebibliography}
